Optimality Conditions for Weak and Strong Local Extrema in Infinite Horizon Optimal Control Problems

In this paper we summarize our results in infinite horizon optimal control. We present optimality conditions for weak local minimizer in the framework of weighted functions. Moreover we formulate the Pontryagin Maximum Principle for strong local minimizer for trajectories converging at infinity. The considered problems, the requirements and the results depend on the choice of the function space.

==> 1-Einleitung.tex <==
\section{Einleitung}
Die Optimale Steuerung mit unendlichem Zeithorizont liefert die wesentliche Grundlage zur Formulierung und Untersuchung
von Aufgaben in der "Okonomischen Wachstumstheorie.
Im Rahmen der "Okonomischen Wachstumstheorie werden z.\,B. die Interaktionen sich "uberschneidender Generationen oder die Determinanten 
des wirtschaftlichen Wachstums,
insbesondere unter sich "andernden Umweltbedingungen wie globaler Erw"armung oder ersch"opfenden nat"urlichen Ressourcen, untersucht.
Aufgrund der Langlebigkeit der wirtschafts- und sozialpolitischen Entscheidungen muss dabei die Frage nach einem geeigneten 
Planungszeitraum aufgeworfen werden:
Jeder endliche Zeithorizont stellt die Forderung nach einer ad"aquaten Ausgangslage f"ur die nachfolgenden Generationen.
Um die Beachtung aller nachfolgenden Generationen zu gew"ahrleisten,
wird der Zeitrahmen in Form des unendlichen Zeithorizontes idealisiert (Arrow \& Kurz \cite{Arrow}). \\[2mm]
Der erste mathematische Beitrag zu einem Problem mit unbeschr"anktem Zeitintervall besteht in einer Aufgabe der Variationsrechnung,
in der die Frage nach der optimalen Sparquote einer Gesellschaft behandelt wird (Ramsey \cite{Ramsey}).
Bei n"aherer Betrachtung entsteht in diesem Problem nicht nur die Aufgabe die Optimalit"atsbedingungen "uber dem unendlichen Zeithorizont zu formulieren,
sondern insbesondere die Gestalt der Transversalit"atsbedingungen im Unendlichen zu charakterisieren. 
Diese Fragestellung stellt allerdings eine schwerwiegende Herausforderung dar,
denn die bekannten Resultate k"onnen nicht einfach "ubernommen und die bekannten Methoden k"onnen nicht
unmittelbar an das unbeschr"ankte Intervall angepasst werden. \\[2mm]
Von den wenigen uns bekannten Resultaten,
die den unendlichen Zeithorizont nicht auf ein endliches Intervall reduzieren,
z"ahlen wir die Arbeiten von Brodskii \cite{Brodskii} und Pickenhain \cite{Pickenhain} auf.
In diesen Beitr"agen werden auf der Basis von schwachen lokalen Variationen und der Anwendung geeigneter funktionalanalytischer Methoden
notwendige Optimalit"atsbedingungen f"ur Steuerungsprobleme mit unendlichem Zeithorizont erzielt.
In \cite{Brodskii} wird eine sehr allgemeine Aufgabenklasse mit Zustandsbeschr"ankungen und Randbedingungen im Unendlichen betrachtet.
Aufgrund der Wahl des Raumes der messbaren und beschr"ankten Funktionen f"uhrt der funktionalanalytische Rahmen allerdings
zu keiner ``"asthetischen'' Darstellung der Adjungierten.
Demgegen"uber bezieht sich die Arbeit \cite{Pickenhain} auf Aufgaben mit eindimensionalen linearen Nebenbedingungen und mit freiem rechten Endpunkt.
Der innovative Beitrag in \cite{Pickenhain} ist die Wahl des gewichteten Sobolev-Raumes,
in dessen Rahmen die ``nat"urlichen'' Transversalit"atsbedingungen in gewisser Weise Eigenschaften der Elemente dieser R"aume sind.
An der Arbeit \cite{Pickenhain} ist jedoch anzumerken,
dass sich die angewandte Beweismethode auf linear-quadratische Aufgaben fokussiert.
Die Anwendbarkeit der Beweisstrategie im Fall von Aufgaben mit einer nichtlinearen Dynamik ist offen. \\
In dieser Arbeit pr"asentieren wir das Pontrjaginsche Maximumprinzip f"ur Steuerungsprobleme mit unendlichem Zeithorizont.
Dabei erweitern wir die mehrfachen Nadelvariationen nach Ioffe \& Tichomirov \cite{Ioffe} f"ur das unbeschr"ankte Zeitintervall.
Weiterhin gehen wir auf Randbedingungen im Unendlichen und auf Zustandsbeschr"ankungen "uber dem unendlichen Zeithorizont ein.
Zur Aufgabenklasse mit Zustandsbeschr"ankungen existieren bisher nur sehr wenige Beitr"age.
Wir erarbeiten einen Zugang im Rahmen der stetigen Funktionen, die im Unendlichen einen Grenzwert besitzen.
Die Anforderung, die wir dabei an die Aufgabe stellen,
sind verwandt mit denen bei Brodskii \cite{Brodskii}.
Die Darstellung der notwendigen Optimalit"atsbedingungen besitzen wegen diesem Zugang eine enge Verwandtschaft mit dem Maximumprinzip f"ur Aufgaben mit endlichem
Zeitintervall. \\[2mm]
Ein sehr wichtiges und zentrales Anliegen dieser Arbeit ist die Einordnung der Aufgabe mit unendlichem Zeithorizont in die Theorie der Optimalen Steuerung.
Wir gehen dazu auf die h"aufig angewandte Approximation mit endlichem Zeithorizont und auf die R"uckf"uhrung auf ein endliches Zeitintervall mittels der
Substitution der Zeit ein.
Es zeigt sich,
dass einerseits bei der Approximation der vollst"andige Satz an notwendigen Optimalit"atsbedingungen verloren geht
und andererseits die Substitution der Zeit den unendlichen Zeithorizont in eine Singularit"at in der Aufgabe mit endlichem Zeitintervall "uberf"uhrt.
Umgekehrt k"onnen wir wiederum zeigen,
dass das Pontrjaginsche Maximumprinzip im Kapitel zu starken lokalen Minimalstellen "uber einem endlichen Zeitintervall eine direkte Konsequenz der Ergebnisse
dieses Kapitels darstellt.
Somit sind die Steuerungsprobleme "uber endlichem Zeithorizont eine echte Unterklasse der Steuerungsprobleme mit unendlichem Zeithorizont.
Die Untersuchungen liefern damit nicht nur technisch bez"uglich der Nadelvariationsmethode und der Behandlung der Zustandsbeschr"ankungen innovative Beitr"age,
sondern es zeigt sich viel mehr die besondere Qualit"at der Aufgabe mit unendlichem Zeithorizont als eine echte Verallgemeinerung der Aufgabenklasse mit
endlichem Zeithorizont.
